Hierarchical Programmatic Reinforcement Learning via Learning to Compose Programs

Aiming to produce reinforcement learning (RL) policies that are human-interpretable and can generalize better to novel scenarios, Trivedi et al. (2021) present a method (LEAPS) that first learns a program embedding space to continuously parameterize diverse programs from a pre-generated program dataset, and then searches for a task-solving program in the learned program embedding space when given a task. Despite the encouraging results, the program policies that LEAPS can produce are limited by the distribution of the program dataset. Furthermore, during searching, LEAPS evaluates each candidate program solely based on its return, failing to precisely reward correct parts of programs and penalize incorrect parts. To address these issues, we propose to learn a meta-policy that composes a series of programs sampled from the learned program embedding space. By learning to compose programs, our proposed hierarchical programmatic reinforcement learning (HPRL) framework can produce program policies that describe out-of-distributionally complex behaviors and directly assign credits to programs that induce desired behaviors. The experimental results in the Karel domain show that our proposed framework outperforms baselines. The ablation studies confirm the limitations of LEAPS and justify our design choices.

==> figure/karel_env.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.1475\textwidth}
    \centering
    \includegraphics[trim=30 16 30 45, clip,height=\textwidth]{figure/env_figure/stairClimber_single.pdf}
    \SmallCaption{\textsc{StairClimber}}
    \end{subfigure}
    \begin{subfigure}[b]{0.1475\textwidth}
    \centering
    \includegraphics[trim=30 16 30 45, clip,height=\textwidth]{figure/env_figure/fourCorners_single.pdf}
    \SmallCaption{\textsc{FourCorner}}
    \end{subfigure}
    \begin{subfigure}[b]{0.1475\textwidth}
    \centering
    \includegraphics[trim=30 16 30 45, clip,height=\textwidth]{figure/env_figure/topOff_single.pdf}
    \SmallCaption{\textsc{TopOff}}
    \end{subfigure}
    \begin{subfigure}[b]{0.1475\textwidth}
    \centering
    \includegraphics[trim=30 16 30 45, clip,height=\textwidth]{figure/env_figure/maze_single.pdf}
    \SmallCaption{\textsc{Maze}}
    \end{subfigure}
    \begin{subfigure}[b]{0.23325\textwidth}
    \centering
    \includegraphics[trim=50 0 50 40, clip,width=\textwidth]{figure/env_figure/cleanHouse_single.pdf}
    \SmallCaption{\textsc{CleanHouse}}
    \end{subfigure}
    \begin{subfigure}[b]{0.1475\textwidth}
    \centering
    \includegraphics[trim=30 16 30 45, clip,height=\textwidth]{figure/env_figure/harvester_single.pdf}
    \SmallCaption{\textsc{Harvester}}
    \end{subfigure}
    \caption[]{
    \textbf{The Karel tasks}: 
    The six tasks feature a set of diverse, goal-oriented, programmatic behaviors, 
    requiring the agent to navigate through the gridworld 
    and interact with markers (in diamond shape).
    The tasks are further described in~\mysecref{sec:env details} 
    with desired behaviors visualized
    in~\myfig{fig:karel both env}.}
    \label{fig:karel env}
\end{figure*}

==> table/ablation_program_len.tex <==
\begin{table}
\centering
% \scriptsize
\caption[]{Mean return (standard deviation) achieved by composing programs with different maximum lengths, 
evaluated over five random seeds.}
%\ra{1.3}
\scalebox{0.9}{\begin{tabular}{@{}ccc@{}}\toprule
Program Length & \textsc{StairClimber} & \textsc{FourCorner}\\
\cmidrule{1-3}
18  & 0.25 & 0.44 \\
36  & 1.0  & 0.58 \\
\bottomrule
\end{tabular}}
\label{table:ablation_len_program}
\end{table}

==> table/ablation_program_num.tex <==
\begin{table}
\centering
% \scriptsize
\caption[]{Mean return (standard deviation) achieved by composing different numbers of programs, 
evaluated over five random seeds.}
%\ra{1.3}
\scalebox{0.9}{\begin{tabular}{@{}ccc@{}}\toprule
\# Programs & \textsc{StairClimber} & \textsc{FourCorner}\\
\cmidrule{1-3}
1  & 0.25 & 0.44 \\
3  & 1.0  & 0.58 \\
5  & 0.91 & 0.66 \\
7  &  & \\
10 & 1.0  & 0.78 \\
\bottomrule
\end{tabular}}
\label{table:ablation_program_num}
\end{table}

==> table/ablation_rl_algo.tex <==
\begin{table}
\centering
% \scriptsize
\caption[]{Mean return (standard deviation) achieved by learning the meta-policy using different RL algorithms, 
evaluated over five random seeds.}
%\ra{1.3}
\scalebox{0.9}{\begin{tabular}{@{}ccc@{}}\toprule
RL Algorithm & \textsc{CleanHouse} & \textsc{Seeder}\\
\cmidrule{1-3}
PPO~\cite{schulman2017proximal}  & 1.0 \pm 0.00 & 0.58 \pm 0.10\\
SAC~\cite{haarnoja18b}  & 1.0 \pm 0.00 & 0.25 \pm 0.11\\
\bottomrule
\end{tabular}}
\label{table:ablation_rl_algo}
\end{table}

==> table/karel_hard_recon.tex <==


\begin{table*}
\centering
% \scriptsize
\caption[]{Mean return and standard deviation of all methods across the \textsc{Karel-Hard} problem set, 
evaluated over five random seeds.}
%\ra{1.3}
\scalebox{0.9}{\begin{tabular}{@{}ccccc@{}}\toprule
Method % & \textsc{Delivery} 
& \textsc{DoorKey} & \textsc{OneStroke} & \textsc{Seeder} & \textsc{Snake}\\
\cmidrule{2-5}
LEAPS % & \textbf{0.50} \pm 0.00 
& \textbf{0.50} \pm 0.00 & 0.65 \pm 0.24 & 0.51 \pm 0.06 & 0.23 \pm 0.10 \\
LEAPS-ours % & \textbf{0.50} \pm 0.00 
& \textbf{0.50} \pm 0.00 & 0.68 \pm 0.11 & 0.56 \pm 0.00 & 0.28 \pm 0.08 \\
\midrule
{\method\\-SAC}
& \textbf{0.50} \pm 0.00 & \textbf{0.73} \pm 0.12 & 0.25 \pm 0.11 & 0.13 \pm 0.08 \\
{\method\\-PPO} % & \textbf{0.50} \pm 0.00 
& \textbf{0.50} \pm 0.00 & \textbf{0.7*} \pm 0.00 & \textbf{0.58} \pm 0.10 & \textbf{0.33} \pm 0.12 \\
\bottomrule
\end{tabular}}
\label{table:karel_hard}
\end{table*}

==> table/sub_programs_v2.tex <==

\begin{table}
\centering
% \scriptsize
%\ra{1.3}
\caption[]{Mean reward for meta-policy methods using different sub-program length constraints across Karel tasks}
\scalebox{0.8}{\begin{tabular}{@{}ccccccc@{}}\toprule
& \textsc{StairClimber} & \textsc{FourCorner} & \textsc{TopOff} & \textsc{Maze} & \textsc{CleanHouse} & \textsc{Harvester}\\
\cmidrule{1-7}
5  & 1.0 & 0.91         & 0.38        & 1.0 & 0.1           & 0.66 \\
10 & 1.0 & \textbf{1.0} & textbf{0.4} & 1.0 & \textbf{0.36} & \textbf{0.78} \\
\bottomrule
\end{tabular}}
\label{table:ablation-sub-program-lengths}
\end{table}



==> text/algo.tex <==
\begin{algorithm}[H]
\caption{Hierarchical Programmatic Reinforcement Learning} 
\label{alg:algo}
\textbf{Input}: Program Dataset $D_{program}$, VAE Training Epoch $N_{epoch}$, Meta-Policy Training Step $T_{meta}$, Program Synthesis Step $|H|$\\
\textbf{Output}: Task Solving Program $\mathcal{P}$
\begin{algorithmic}[1]
  \STATE Initialize the program encoder $q_\phi$ and decoder $p_\theta$, compression encoder $f_\omega$ and decoder $g_\psi$, neural execution policy $\pi$.
  \FOR{$\text{epoch}$ in range(1, $N_{epoch}$)}
    \FOR{program $\rho$ in $D_{program}$}
    \STATE    $z = f_\omega(q_\phi(\rho))$
    \STATE    $\hat{\rho} = p_\theta(g_\psi(z))$ 
    \STATE    compute $\mathcal{L}_{total} = \mathcal{L}^P_{\theta, \phi, \omega, \phi}(\rho) + \lambda\mathcal{L}^L_{\pi}(\rho, \pi)$
    \STATE    fit $\phi, \omega, \psi, \theta, \pi$ to minimize $\mathcal{L}_{total}$
    \ENDFOR
  \ENDFOR
  \STATE Initialize a meta-policy $\pi_{meta}$
  \STATE Load and fix $p_\theta, g_\psi$ for Meta-Policy Training
  \FOR{Training Episode in range(1, $T_{meta}/|H|$)}
    \STATE Receive initial state $s^1$ from the Karel environment
    \FOR{i in range(1, $|H|$)}
      \STATE $z_i = \pi_{meta}(s^i)$
      \STATE $\rho_i = p_\theta(g_\psi(z_i))$
      \STATE Interact with the environment by \textsc{EXEC}($\rho_i$)
      \STATE Receive $[s^i_1, ..., s^i_T]$ and $[r^i_1, ..., r^i_{T_i}]$
      \STATE $r^{i+1} = \sum_{t=1}^{T^i} r^i_t$
      \STATE $s^{i+1} = [s^i_1, s^i_2, ..., s^i_{T_i}][-1]$ 
    \ENDFOR
    \STATE Calculate $\mathcal{J}_{\pi_{meta}}$ based on the collected $(s^i, z^i, r^{i+1}, s^{i+1})$
    \STATE fit $\pi_{meta}$ to maximize $\mathcal{J}_{\pi_{meta}}$
  \ENDFOR
\end{algorithmic}
\end{algorithm}
